The Neural Testbed: Evaluating Joint Predictions

Predictive distributions quantify uncertainties ignored by point estimates. This paper introduces The Neural Testbed: an open-source benchmark for controlled and principled evaluation of agents that generate such predictions. Crucially, the testbed assesses agents not only on the quality of their marginal predictions per input, but also on their joint predictions across many inputs. We evaluate a range of agents using a simple neural network data generating process. Our results indicate that some popular Bayesian deep learning agents do not fare well with joint predictions, even when they can produce accurate marginal predictions. We also show that the quality of joint predictions drives performance in downstream decision tasks. We find these results are robust across choice a wide range of generative models, and highlight the practical importance of joint predictions to the community.

==> NT NeurIPS 2D/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Including Packages
\usepackage{color}
\usepackage{algorithm}
\usepackage{algorithmic}
% \usepackage{algpseudocode}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{lmodern}
\usepackage{array}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage[mathscr]{eucal}
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{psfrag}
\usepackage{color}
\usepackage{here}
\usepackage{wasysym}
\usepackage{enumitem}
% \usepackage[dvipsnames, table]{xcolor}
% \usepackage{caption}
\usepackage{subcaption}
\usepackage{amsthm}
\usepackage{lipsum}
\usepackage{todonotes}
\usepackage{tabulary}
\usepackage{pifont}
\usepackage{outlines}

\newtheorem{theorem} {Theorem}
\newtheorem{conjecture} {Conjecture}
\newtheorem{proposition} {Proposition}
\newtheorem{lemma} {Lemma}
\newtheorem{corollary} {Corollary}
\newtheorem{assumption} {Assumption}
\newtheorem{definition} {Definition}
\newtheorem{property} {Property}
\newtheorem{axiom} {Axiom}
\newtheorem{fact} {Fact}
\newtheorem{remark} {Remark}
\newtheorem{example} {Example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Setting up macro shortcuts
\newcommand{\Exp}{\mathds{E}}
\newcommand{\Expk}{\mathds{E}_{k}}
\newcommand{\Prob}{\mathds{P}}
\newcommand{\Real}{\mathds{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\Rmax}{R_{\rm max}}
\newcommand{\riskyopt}{\succcurlyeq_{\rm ro}}
\newcommand{\cid}{\succcurlyeq_{\rm CID}}
\newcommand{\so}{\succcurlyeq_{\rm so}}
\newcommand{\single}{\succcurlyeq_{\rm sc}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\dtrain}{\mathcal{D}_{\mathrm{train}}}
\newcommand{\ENN}{{\tt ENN}}
\newcommand{\KL}{\mathbf{d}_{\mathrm{KL}}}
\newcommand{\KLBAR}{\overline{\mathbf{d}}_{\mathrm{KL}}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}


\newcommand{\reals}{\mathbf{R}}
\newcommand{\environment}{\mathcal{E}}
\newcommand{\proxy}{\tilde{\mathcal{E}}}
\newcommand{\KLp}{\mathbf{\tilde{d}}_{\textrm{KL}}}

\newcommand{\ass}{\hspace{-1mm} = \hspace{-0.5mm} \mathbf{\cdot} \hspace{0.5mm}}
\newcommand{\tick}{\textcolor{ForestGreen}{\ding{51}}}
\newcommand{\ok}{\textcolor{Dandelion}{\ding{108}}}
\newcommand{\cross}{\textcolor{BrickRed}{\ding{55}}}
\newcommand{\fillpara}{\vspace{22mm}}
\DeclareMathOperator*{\softmax}{softmax}

\definecolor{ian_highlight}{RGB}{100, 2, 2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Weird algo stuff (Comment out if you don't want the for loop lines)

\errorcontextlines\maxdimen

% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
\makeatletter
% start with some helper code
% This is the vertical rule that is inserted
    \newcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em}\thealgruleextra\vrule height \thealgruleheight depth \thealgruledepth}}%
% its height and depth need to be adjustable
\newcommand*{\thealgruleextra}{}
\newcommand*{\thealgruleheight}{.75\baselineskip}
\newcommand*{\thealgruledepth}{.25\baselineskip}

\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0% is there anything to print
        \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
            % do nothing
        \else
            \unskip
            \addvspace{-1pt}% FUDGE to make the rules line up
            % draw a rule for each indent level
            \ALG@printindent@tempcnta=1
            \loop
                \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
                \advance \ALG@printindent@tempcnta 1
            \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
            \repeat
        \fi
    \fi
    }%
\usepackage{etoolbox}
% the following line injects our new indent handling code in place of the default spacing
% \patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\makeatother

% the required height and depth are set by measuring the content to be shown
% this means that the content is processed twice
\newbox\statebox
\newcommand{\myState}[1]{%
    \setbox\statebox=\vbox{#1}%
    \edef\thealgruleheight{\dimexpr \the\ht\statebox+1pt\relax}%
    \edef\thealgruledepth{\dimexpr \the\dp\statebox+1pt\relax}%
    \ifdim\thealgruleheight<.75\baselineskip
        \def\thealgruleheight{\dimexpr .75\baselineskip+1pt\relax}%
    \fi
    \ifdim\thealgruledepth<.25\baselineskip
        \def\thealgruledepth{\dimexpr .25\baselineskip+1pt\relax}%
    \fi
    %\showboxdepth=100
    %\showboxbreadth=100
    %\showbox\statebox
    \State #1%
    %\State \usebox\statebox
    %\State \unvbox\statebox
    %reset in case the next command is not wrapped in \myState
    \def\thealgruleheight{\dimexpr .75\baselineskip+1pt\relax}%
    \def\thealgruledepth{\dimexpr .25\baselineskip+1pt\relax}%
}
% end vertical rule patch for algorithmicx


==> NT NeurIPS 2D/testbed_pseudocode.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PSEUDOCODE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Testbed Pseudocode}
\label{app:testbed_pseudo_code}

We present the testbed pseudocode in this section. Specifically, Algorithm~\ref{alg:neural-testbed} is the pseudocode for our neural testbed, and Algorithm~\ref{alg:mc-estimation} is an approach to estimate the likelihood of a test data $\tau$-sample conditioned on an agent's belief, based on the standard Monte-Carlo estimation.
%
% and Algorithm~\ref{alg:rp-estimation} are two different approaches to estimate the likelihood of a test data $\tau$-sample conditioned on an agent's belief. Algorithm~\ref{alg:mc-estimation} is based on the standard Monte-Carlo estimation, while Algorithm~\ref{alg:rp-estimation} adopts a random partitioning approach. 
% As a rule of thumb, we recommend the users to use Algorithm~\ref{alg:mc-estimation} for $\tau < 10$ and Algorithm~\ref{alg:rp-estimation}  with a feature dimension between $5$ and $10$ for $\tau \geq 10$.
The presented testbed pseudocode works for any prior $\Prob(\environment \in \cdot)$ over the environment and any input distribution $P_X$, including the ones described in Section \ref{sec:generative}.
We also release full code and implementations in Appendix~\ref{app:code}.

% We present the testbed pseudocode in this section. Specifically, Algorithm~\ref{alg:neural-testbed} is the pseudocode for our neural testbed, and Algorithm~\ref{alg:mc-estimation} and Algorithm~\ref{alg:rp-estimation} are two different approaches to estimate the likelihood of a test data $\tau$-sample conditioned on an agent's belief. Algorithm~\ref{alg:mc-estimation} is based on the standard Monte-Carlo estimation, while Algorithm~\ref{alg:rp-estimation} adopts a random partitioning approach. 
% % As a rule of thumb, we recommend the users to use Algorithm~\ref{alg:mc-estimation} for $\tau < 10$ and Algorithm~\ref{alg:rp-estimation}  with a feature dimension between $5$ and $10$ for $\tau \geq 10$.
% The presented testbed pseudocode works for any prior $\Prob(\environment \in \cdot)$ over the environment and any input distribution $P_X$, including the ones described in Section \ref{sec:generative}.
% We also release full code and implementations at \github.
% we also discuss some core technical issues in the neural testbed design. Specifically,
% % Appendix~\ref{app:likelihood_estimation} discusses how to estimate the likelihood of an agent's belief distribution;
% Appendix~\ref{app:evaluation_real_data} discusses how to extend the testbed to agent evaluation on real data and Appendix~\ref{app:experiment_parameters} explains our choices of experiment parameters.



\begin{algorithm}
\caption{Neural Testbed}
\label{alg:neural-testbed}
% \setstretch{1.1}
\begin{algorithmic}
\REQUIRE the testbed requires the following inputs
\begin{enumerate}
\item prior distribution over the environment $\Prob(\environment \in \cdot)$, input distribution $P_X$
\item agent $f_\theta$
\item number of training data $T$, test distribution order $\tau$
\item number of sampled problems $J$, number of test data samples $N$
\item parameters for agent likelihood estimation, as is specified in Algorithm~\ref{alg:mc-estimation} 
% and \ref{alg:rp-estimation}
\end{enumerate}
\vspace{0.3em}
\FOR{$j=1, 2, \ldots, J$}
\vspace{0.3em}
\STATE \textbf{Step 1: sample environment and training data}
    \STATE \hspace{1em} 1. sample environment $\environment \sim \Prob(\environment \in \cdot)$
    \STATE \hspace{1em} 2. sample $T$ inputs $X_0, X_1, \ldots, X_{T-1}$ i.i.d. from $P_X$ \STATE \hspace{1em} 3. sample the training labels
    $Y_1, \ldots, Y_T$ conditionally i.i.d. as
    \[
    Y_{t+1} \sim \Prob \left(Y \in \cdot \middle | \environment, X = X_t \right) \quad \forall t=0, 1, \ldots, T-1
    \]
    \STATE \hspace{1em} 4. choose the training dataset as
    $
    \data_T = \left \{ \left(X_t, Y_{t+1} \right), \, t=0, \ldots, T-1 \right \}$
\vspace{0.3em}
\STATE \textbf{Step 2: train agent}
    \STATE \hspace{1em} train agent $f_{\theta_T}$ based on training dataset $\data_T$
\vspace{0.3em}
\STATE \textbf{Step 3: compute likelihoods}
    \STATE \hspace{1em} \textbf{for} $n=1,2,\ldots, N$ \textbf{do}
        \STATE \hspace{2em} 1. sample $X^{(n)}_{T}, \ldots, X^{(n)}_{T+\tau-1}$ i.i.d. from $P_X$
        \STATE \hspace{2em} 2. generate $Y^{(n)}_{T+1}, \ldots, Y^{(n)}_{T+\tau}$ conditionally independently as
    \[
    Y_{t+1}^{(n)} \sim \Prob \left(Y \in \cdot \middle | \environment, X = X_t^{(n)} \right) \quad \forall t=T, T+1, \ldots, T+\tau-1
    \]
    % the testing dataset is $\tilde{\data}^{(n)}_\tau = \left \{
    % \left ( X_t^{(n)}, Y_{t+1}^{(n)} \right), t=T, \ldots, T+\tau-1
    % \right \}$
    \STATE \hspace{2em} 3. compute the likelihood under the environment $\environment$ as
    \begin{align*}
        \textstyle p_{j,n} = \Prob \left(
        Y_{T+1:T+\tau}^{(n)}\middle | \environment, 
         X_{T:T+\tau-1}^{(n)}
        \right) = \prod_{t=T}^{T+\tau-1} 
        \Pr \left(Y_{t+1}^{(n)} \middle | \environment, X_{t}^{(n)}
        \right)
    \end{align*}
    \STATE \hspace{2em} 4. estimate the likelihood conditioned on the agent's belief 
    \[
    \hat{p}_{j,n} \approx \Prob \left(\hat{Y}_{T+1:T+\tau} = Y_{T+1:T+\tau}^{(n)} \middle | \theta_T,   X_{T:T+\tau-1}^{(n)},  Y_{T+1:T+\tau}^{(n)}  \right) ,\] 
    \STATE \hspace{2em} based on Algorithm~\ref{alg:mc-estimation} 
    % or \ref{alg:rp-estimation} 
    with test data $\tau$-sample 
    $\left(X_{T:T+\tau-1}^{(n)}, Y_{T+1:T+\tau}^{(n)} \right)$. 
    \vspace{0.3em}
\ENDFOR \\
\RETURN $\frac{1}{JN} \sum_{j=1}^J \sum_{n=1}^N \log \left( p_{j,n}/\hat{p}_{j,n} \right)$
\end{algorithmic}
% \setstretch{1}
\end{algorithm}



\begin{algorithm}
\caption{Monte Carlo Estimation of Likelihood of Agent's Belief}
\label{alg:mc-estimation}
\begin{algorithmic}
\REQUIRE the Monte-Carlo estimation requires the following inputs
\begin{enumerate}
    \item trained agent $f_{\theta_T}$ and number of Monte Carlo samples $M$
    \item test data $\tau$-sample $\left(X_{T:T+\tau-1}, Y_{T+1:T+\tau} \right)$
\end{enumerate}
\STATE \textbf{Step 1:} sample $M$ models $\hat{\environment}_1, \ldots, \hat{\environment}_M$ conditionally i.i.d. from $\Prob \left( \hat{\environment} \in \cdot \middle | \theta_T \right)$
\STATE \textbf{Step 2:} estimate $\hat{p}$ as
\[
\hat{p} = \frac{1}{M} \sum_{m=1}^M
\Prob \left(\hat{Y}_{T+1:T+\tau} = Y_{T+1:T+\tau} \middle | \hat{\environment}_m,   X_{T:T+\tau-1},  Y_{T+1:T+\tau}  \right)
\]
\RETURN $\hat{p}$
\end{algorithmic}
\end{algorithm}


In addition to presenting the testbed pseudocode, we also explain our choices of experiment parameters in Appendix~\ref{app:agents}.
To apply Algorithm \ref{alg:neural-testbed}, we need to specify an input distribution $P_X$ and a prior distribution on the environment $\Prob(\environment \in \cdot)$. Recall from Section \ref{sec:generative} that we consider binary classification problems with input dimension $2$. We choose $P_X = N(0, I)$, and we consider three environment priors distinguished by a temperature parameter that controls the signal-to-noise ratio (SNR) regime. We sweep over temperatures in $\{0.01, 0.1, 0.5\}$. The prior distribution $\Prob(\environment \in \cdot)$ is induced by a distribution over MLPs with 2 hidden layers and ReLU activation. The MLP is distributed according to standard Xavier initialization, except that biases in the first layer are drawn from $N(0, \frac{1}{2})$. The MLP outputs two units, which are divided by the temperature parameter and passed through the softmax function to produce class probabilities.
The implementation of this generative model is in our open source code under the path \url{/generative/factories.py}.

We now describe the other parameters we use in the Testbed. In Algorithm \ref{alg:neural-testbed}, we pick the order of predictive distributions $\tau \in \{1, 10\}$, training dataset size $T \in \{1, 3, 10, 30, 100, 300, 1000\}$, number of sampled problems $J = 10$, and number of testing data $\tau$-samples $N = 1000$. To apply Algorithm~\ref{alg:mc-estimation}, we sample 
$M = 1000$ models from the agent.






